Modelling and Refinement in CODA

This paper provides an overview of the CODA framework for modelling and refinement of component-based embedded systems. CODA is an extension of Event-B and UML-B and is supported by a plug-in for the Rodin toolset. CODA augments Event-B with constructs for component-based modelling including components, communications ports, port connectors, timed communications and timing triggers. Component behaviour is specified through a combination of UML-B state machines and Event-B. CODA communications and timing are given an Event-B semantics through translation rules. Refinement is based on Event-B refinement and allows layered construction of CODA models in a consistent way.

==> eptcsdata.tex <==
\providecommand{\firstpage}{36}
\providecommand{\publicationstatus}{John Derrick, Eerke Boiten, Steve Reeves (Eds.):\\
Refinement Workshop 2013\\
EPTCS 115, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.115.3}{10.4204/EPTCS.115.3}}
\pdfoutput=1

